Learning Dynamic Abstract Representations for Sample-Efficient Reinforcement Learning

In many real-world problems, the learning agent needs to learn a problem's abstractions and solution simultaneously. However, most such abstractions need to be designed and refined by hand for different problems and domains of application. This paper presents a novel top-down approach for constructing state abstractions while carrying out reinforcement learning. Starting with state variables and a simulator, it presents a novel domain-independent approach for dynamically computing an abstraction based on the dispersion of Q-values in abstract states as the agent continues acting and learning. Extensive empirical evaluation on multiple domains and problems shows that this approach automatically learns abstractions that are finely-tuned to the problem, yield powerful sample efficiency, and result in the RL agent significantly outperforming existing approaches.

==> todo.tex <==
mention that we're adding code?

add env layouts in supplementary?

hyperparameters in the supplementary:
 In the wumpus world, we use a discount of $\gamma$=0.95, epsilon of 0.95, and epsilon decay of 0.99 for CA+RL, Option-critic, and Q-learning, while a constant epsilon of 0.3 for JIRP as it improved its performance. In the taxi domain, we use a discount of 1.0. We found that an epsilon of 0.4 performed best for JIRP and an epsilon of 1.0 with decay rate of 0.99 performed best for taxi world and office world. In the office world, we use a discount of 0.99. Finally, we use a learning rate of 0.05 in all the experiments. For comparison with JIRP, we also constructed true reward machines as required by the method to train RL agents for all the reward functions of the domains described earlier.
 
 
 we use the same reward function across algorithms 
 sparse as well as non-sparse reward functions
 
  # IMP: 
add about vanilla qlearing + conditional abstractions
add about our method works with continuous domains
each node represents..


why performance low in wumpus
future: discovering options


Clean Citations {{}}

